PECAN: A Deterministic Certified Defense Against Backdoor Attacks

Neural networks are vulnerable to backdoor poisoning attacks, where the attackers maliciously poison the training set and insert triggers into the test input to change the prediction of the victim model. Existing defenses for backdoor attacks either provide no formal guarantees or come with expensive-to-compute and ineffective probabilistic guarantees. We present PECAN, an efficient and certified approach for defending against backdoor attacks. The key insight powering PECAN is to apply off-the-shelf test-time evasion certification techniques on a set of neural networks trained on disjoint partitions of the data. We evaluate PECAN on image classification and malware detection datasets. Our results demonstrate that PECAN can (1) significantly outperform the state-of-the-art certified backdoor defense, both in defense strength and efficiency, and (2) on real back-door attacks, PECAN can reduce attack success rate by order of magnitude when compared to a range of baselines from the literature.

==> tables/xba_res_full.tex <==
\begin{table*}
    \centering
    \caption{Results of \technique and other defense approaches trained on poisoned dataset $\poisoned{D}_3$ when evaluated on the malware test set with malicious triggers, the (original) malware test set without malicious triggers, and  the (original) non-malware test set without malicious triggers.}
    \setlength{\tabcolsep}{2pt}
    \scriptsize
    \begin{tabular}{llllllllll}
    \toprule
       & \multicolumn{3}{c}{Malware test set with triggers}                 & \multicolumn{3}{c}{Malware test set  without triggers}
            & \multicolumn{3}{c}{Non-Malware test set without triggers}\\ 
 \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} 
        Approaches & ASR ($\downarrow$) & Accuracy ($\uparrow$) & Abs. Rate & ASR ($\downarrow$) & Accuracy ($\uparrow$) & Abs. Rate & ASR ($\downarrow$) & Accuracy ($\uparrow$) & Abs. Rate \\ \midrule
        NoDef & 66.37\% (11.21) & 33.63\% (11.21) & N/A & 1.46\% (0.51) & 98.54\% (0.51) & N/A & ~~1.83\% (0.61) & 98.17\% (0.61) & N/A \\ 
        Isolation Forest & 36.33\% (~~7.98) & 63.67\% (~~7.98) & N/A & 0.89\% (0.15) & 99.11\% (0.15) & N/A & 10.68\% (0.50) & 89.32\% (0.50) & N/A \\ 
        HDBSCAN & 64.71\% (10.14) & 35.29\% (10.14) & N/A & 1.46\% (0.81) & 98.54\% (0.81) & N/A & ~~2.29\% (1.00) & 97.71\% (1.00) & N/A \\ 
        Spectral Signature & 65.52\% (12.98) & 34.48\% (12.98) & N/A & 1.52\% (0.80) & 98.48\% (0.80) & N/A & ~~1.94\% (1.31) & 98.06\% (1.31) & N/A \\ 
        MDR & 60.25\% (~~5.42) & 39.75\% (~~5.42) & N/A & 1.42\% (0.47) & 98.58\% (0.47) & N/A & ~~2.29\% (1.05) & 97.71\% (1.05) & N/A \\ 
        Friendly Noise & 58.76\% (~~1.76) & 41.24\% (~~1.76) & N/A & 3.24\% (0.17) & 96.76\% (0.17) & N/A & ~~6.04\% (0.10) & 93.96\% (0.10) & N/A \\ 
        CROWN-IBP & ~~6.58\% (~~2.80) & 29.05\% (~~2.79) & 64.38\% (2.85) & 5.76\% (2.55) & 46.41\% (1.50) & 47.83\% (2.54) & ~~5.62\% (1.38) & 77.67\% (2.36) & 16.71\% (1.29) \\ 
        DPA & 24.87\% & 19.59\% & 55.54\% & 1.97\% & 64.58\% & 33.45\% & ~~7.91\% & 78.96\% & 13.14\% \\ 
        FPA & ~~0.72\% & 34.26\% & 65.02\% & 0.40\% & 61.64\% & 37.96\% & ~~0.02\% & 91.18\% & ~~8.80\% \\ 
        \technique & ~~1.18\% & 21.39\% & 77.43\% & 0.71\% & 34.38\% & 64.91\% & ~~5.17\% & 53.86\% & 40.96\% \\ 
        \bottomrule
    \end{tabular}
    \label{tab:xba_res_full}
\end{table*}

\begin{table*}
    \centering
    \caption{Results of \technique and FPA trained on poisoned dataset $\newdthree$ when evaluated on the malware test set with malicious triggers, the (original) malware test set without malicious triggers, and  the (original) non-malware test set without malicious triggers.}
    \setlength{\tabcolsep}{2pt}
    \small
    \begin{tabular}{llllllllll}
    \toprule
       & \multicolumn{3}{c}{Malware test set with triggers}                 & \multicolumn{3}{c}{Malware test set  without triggers}
            & \multicolumn{3}{c}{Non-Malware test set without triggers}\\ 
 \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} 
        Approaches & ASR ($\downarrow$) & Accuracy ($\uparrow$) & Abs. Rate & ASR ($\downarrow$) & Accuracy ($\uparrow$) & Abs. Rate & ASR ($\downarrow$) & Accuracy ($\uparrow$) & Abs. Rate \\ \midrule
        FPA & 0.28\% & 13.10\% & 86.61\% &
0.25\% & 15.71\% & 84.04\% &
0.05\% & 77.31\% & 22.64\% \\ 
        \technique & 0.49\% & 26.99\% & 72.52\% &
0.12\% & 34.34\% & 65.54\% &
5.16\% & 54.33\% & 40.52\% \\ 
        \bottomrule
    \end{tabular}
    \label{tab:xba_res_fpa_full}
\end{table*}
